Helion: Enabling a Natural Perspective of Home Automation

Security researchers have recently discovered significant security and safety issues related to home automation and developed approaches to address them. Such approaches often face design and evaluation challenges which arise from their restricted perspective of home automation that is bounded by the IoT apps they analyze. The challenges of past work can be overcome by relying on a deeper understanding of realistic home automation usage. More specifically, the availability of natural home automation scenarios, i.e., sequences of home automation events that may realistically occur in an end-user's home, could help security researchers design better security/safety systems. This paper presents Helion, a framework for building a natural perspective of home automation. Helion identifies the regularities in user-driven home automation, i.e., from user-driven routines that are increasingly being created by users through intuitive platform UIs. Our intuition for designing Helion is that smart home event sequences created by users exhibit an inherent set of semantic patterns, or naturalness that can be modeled and used to generate valid and useful scenarios. To evaluate our approach, we first empirically demonstrate that this naturalness hypothesis holds, with a corpus of 30,518 home automation events, constructed from 273 routines collected from 40 users. We then demonstrate that the scenarios generated by Helion are reasonable and valid from an end-user perspective, through an evaluation with 16 external evaluators. We further show the usefulness of Helion's scenarios by generating 17 home security/safety policies with significantly less effort than existing approaches. We conclude by discussing key takeaways and future research challenges enabled by Helion's natural perspective of home automation.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

This paper initiates a paradigm shift in home automation security analysis.
%, both in terms of {\em what} is analyzed and {\em how}.
We first argue for the analysis of user-driven routines for a practical characterization of home automation.
We then hypothesize that user-driven home automation is natural and hence predictable, and moreover, could lead to useful predictions for security.
We build \tool, a framework that models user-driven home automation sequences using \ngram language models, and validate our hypothesis by demonstrating the naturalness of our {\sf HOME} corpus, relative to natural language and software corpora.
Finally, we explore compelling security use-cases of \tool, which motivate future research in this exciting new direction.

==> sequence_length.tex <==
%\section{Experiment for Deriving Sequence Length}
%\label{app:sequence_length}

%Figure~\ref{fig:sequence_length} shows the plot of the cross-entropy of our model with 10-fold cross validation, for $n=3$, and varying sequence length.
%We choose 20 as it shows average performance in terms of cross-entropy.



==> tables/user_routines.tex <==
\begin{table}[t]
\centering
\scriptsize
\vspace{-0.4cm}
\caption{{\small Some examples routines created by users.}}
\label{tbl:user_routines}
\begin{tabular}{l|l}
\Xhline{2\arrayrulewidth}
{\bf No.}& {\bf Routine}\\
\Xhline{2\arrayrulewidth}
1 & If the air quality is low, switch the Air Purifier ON\\
2 & If the temperature is low, change the thermostat mode to auto.\\
3 & If smoke is detected, trigger the alarm. \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\vspace{-0.3cm}
\end{table}


